Robust Subgraph Generation Improves Abstract Meaning Representation Parsing

The Abstract Meaning Representation (AMR) is a representation for open-domain rich semantics, with potential use in fields like event extraction and machine translation. Node generation, typically done using a simple dictionary lookup, is currently an important limiting factor in AMR parsing. We propose a small set of actions that derive AMR subgraphs by transformations on spans of text, which allows for more robust learning of this stage. Our set of construction actions generalize better than the previous approach, and can be learned with a simple classifier. We improve on the previous state-of-the-art result for AMR parsing, boosting end-to-end performance by 3 F$_1$ on both the LDC2013E117 and LDC2014T12 datasets.

==> discussion.tex <==

Our initial assumption (which we suspect would be shared by many researchers with a background in structured prediction) was that the main area deserving further attention in AMR parsing is predicting the edges in the unreliably-aligned, cyclic, non-projective graphs of AMR (i.e., SRL++).
This intuition follows naturally from an analogy to syntactic dependency parsing.
We spent months testing novel structure-prediction algorithms and training regimes to capture aspects of the non-projective cyclic graphs, only to find that the careful application of an MST variant presented in \newcite{2014flanigan-amr} set an extremely strong baseline for the SRL++ task, and our gains were negligible to non-existent.
